CornerFormer: Boosting Corner Representation for Fine-Grained Structured Reconstruction

Structured reconstruction is a non-trivial dense prediction problem, which extracts structural information (\eg, building corners and edges) from a raster image, then reconstructs it to a 2D planar graph accordingly. Compared with common segmentation or detection problems, it significantly relays on the capability that leveraging holistic geometric information for structural reasoning. Current transformer-based approaches tackle this challenging problem in a two-stage manner, which detect corners in the first model and classify the proposed edges (corner-pairs) in the second model. However, they separate two-stage into different models and only share the backbone encoder. Unlike the existing modeling strategies, we present an enhanced corner representation method: 1) It fuses knowledge between the corner detection and edge prediction by sharing feature in different granularity; 2) Corner candidates are proposed in four heatmap channels w.r.t its direction. Both qualitative and quantitative evaluations demonstrate that our proposed method can better reconstruct fine-grained structures, such as adjacent corners and tiny edges. Consequently, it outperforms the state-of-the-art model by +1.9\%@F-1 on Corner and +3.0\%@F-1 on Edge.

==> texts/tables/table_feature_pass.tex <==
\begin{table}[!t]
    \centering
    \small
    \caption{
    }
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 3pt
	    \begin{tabu}{@{\;} lc@{\quad\;\;}ccc@{\;}}
	        \addlinespace
	        \toprule
	        % {Eval Type } & \multicolumn{3}{c}{Edge} &  \multicolumn{3}{c}{Region} \\
	        % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
	        Feature Extractor &Layer& Corner & Edge &Region \\
	        \midrule
	        Last-layer &1& 87.2 & 76.6 & 68.5   \\
	        MLP  &3&  87.7 & 76.6 & 69.8   \\
	        Learnable &3& 87.7 & 76.9 & 70.8 \\
    	    \bottomrule
	    \end{tabu}
	}
    \label{tab:feature_transfer}
\end{table}

==> texts/tables/table_gt.tex <==
\begin{table}[!t]
    \centering
    \small
    \caption{
    \vspace{-1em}
    }
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 3pt
	    \begin{tabu}{@{\;} cc ccc@{\;}}
	        \addlinespace
	        \toprule
	        FN Corners Enhence & FN Edges Prediction  & Corner & Edge & Region \\
	        \midrule
	         &   & 85.9 & 74.5 & 63.0  \\ 
	      \cmark &   & 87.2 & 75.5 & 68.5 \\ 
            \cmark   & \cmark  & 87.7 & 76.9 & 70.8 \\ 
        	\bottomrule
	    \end{tabu}
	}
    \label{tab:gt}
\end{table}

==> texts/tables/table_indoor.tex <==
\begin{table}[!h]
    \centering
    \small
    \caption{
    }
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 3pt
	    \begin{tabu}{@{\;} l@{\quad\;\;}ccc@{\;}}
	        \addlinespace
	        \toprule
	        % {Eval Type } & \multicolumn{3}{c}{Edge} &  \multicolumn{3}{c}{Region} \\
	        % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
	        Method & Corner & Edge &Region \\
         \midrule
	        \midrule
	        HEAT & 91.7 & 83.7 & \textbf{93.7}   \\
	        CornerFormer+D &  \textbf{92.2} & \textbf{84.5} & 93.4   \\
	        CornerFormer & 91.1 & 82.7 & 92.2  \\
    	    \bottomrule
	    \end{tabu}
	}
    \label{tab:indoor}
\end{table}
% % heat 0.923	0.912	corner f1 0.917	
% 0.852	0.822	edge_f1 0.837	
% 0.947	0.928	region_f10.937
% % ours corners - precision: 0.938 recall: 0.907 f_score: 0.922
% edges - precision: 0.864 recall: 0.826 f_score: 0.845
% regions - precision: 0.937 recall: 0.931 f_score: 0.934
% %ours + mutichannel
% 400 corners - precision: 0.921 recall: 0.902 f_score: 0.911
% edges - precision: 0.840 recall: 0.814 f_score: 0.827
% regions - precision: 0.923 recall: 0.922 f_score: 0.922

==> texts/tables/table_outdoor.tex <==
\begin{table*}[!h]
    \centering
    \small
    \caption{\textbf{Quantitative evaluations on outdoor architecture reconstruction.} Size: the size of the input image. Neural alone: using neural network system alone for true or with heuristic method. Joint: the edge prediction is trained end-to-end with corner detection.
    The colors \first{cyan} and \second{orange} mark the top-two results with different image sizes. 
    }
    \vspace{-1em}
    % \resizebox{\textwidth}{!}
    {
        \tabcolsep 5pt
	    \begin{tabu}{@{\;} lccc @{\quad\;\;\;\;}  ccccccccc@{\;}}
	        \addlinespace
	        \toprule
	       % {Data Type} & \multicolumn{10}{c}{ Outdoor Satellite Images}  \\ 
	        \multicolumn{4}{l}{Evaluation Type} &  \multicolumn{3}{c}{Corner} &  \multicolumn{3}{c}{Edge} &  \multicolumn{3}{c}{Region} \\
	        \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
	        {Method} & Size & Fully-neural & Joint &  Prec & Recall & F-1 & Prec & Recall & F-1 & Prec & Recall & F-1  \\
	        \midrule
	        IP~\cite{IP} & 256 & - & - &  - & - & 74.5 & - & - & 53.1 & - & - & 55.7 \\
	        Exp-Cls~\cite{expcls} & 256 & - & - &  \second{92.2} & 75.9 & 83.2 & 75.4 & 60.4 & 67.1 & 74.9 & 54.7 & 63.5 \\
	       % \midrule
	       %\hdashline
	        ConvMPN~\cite{ConvMPN} & 256 & \cmark & - &  78.0 & 79.7 & 78.8 & 57.0 & 59.7 & 58.1 & 52.4 & 56.5 & 54.4  \\ % 350 test set
	        HAWP~\cite{HAWP} & 256 & \cmark & \cmark &  90.9 & 81.2 & 85.7 & 76.6 & 68.1 & 72.1 & 74.1 & 55.4 & 63.4 \\
	        LETR~\cite{LETR} & 256 & \cmark & \cmark & 87.8 & 74.8 & 80.8 & 59.7 & 58.6 & 59.1 & 68.3 & 48.7 & 56.8 \\
	        HEAT~\cite{HEAT} & 256 & \cmark & \cmark & 91.7 & \second{83.0} & \second{87.1} & \second{80.6} & \second{72.3} & \second{76.2} & \second{76.4} & \second{65.6} & \second{70.6} \\
            \ourmethodtable & 256 & \cmark & \cmark & \first{94.1} & \first{84.5} & \first{89.0} & \first{83.8} & \first{75.1} & \first{79.2} & \first{77.8} & \first{66.9} & \first{71.9}  \\
	        \midrule
	        HAWP~\cite{HAWP} & 512 & \cmark & \cmark & 90.6 & 83.7& 87.0& 78.8 & 72.0 & 75.2 & 77.5 & 57.8 & 66.2 \\
	        LETR~\cite{LETR} & 512 & \cmark & \cmark & 90.3 & 79.7 & 84.7 & 64.0 & 71.6 & 67.6 & 77.1 & 62.6 & 69.1 \\
            HEAT~\cite{HEAT} & 512 & \cmark & \cmark & \second{90.7} & \second{86.7} & \second{88.7} & \second{82.2} & \second{77.4} & \second{79.7} & \first{79.6} & \second{69.0} & \second{73.9}  \\
	        \ourmethodtable & 512 & \cmark & \cmark & \first{92.6} & \first{87.8} & \first{90.2} & \first{83.3} & \first{79.4} & \first{81.3} & \second{79.4} & \first{72.8} & \first{76.0}  \\
    	    \bottomrule
	    \end{tabu}
	}
    \label{tab:outdoor-main}
\end{table*}
